Verifying SQL Queries using Theories of Tables and Relations

We present a number of first- and second-order extensions to SMT theories specifically aimed at representing and analyzing SQL queries with join, projection, and selection operations. We support reasoning about SQL queries with either bag or set semantics for database tables. We provide the former via an extension of a theory of finite bags and the latter via an extension of the theory of finite relations. Furthermore, we add the ability to reason about tables with null values by introducing a theory of nullable sorts based on an extension of the theory of algebraic datatypes. We implemented solvers for these theories in the SMT solver cvc5 and evaluated them on a set of benchmarks derived from public sets of SQL equivalence problems.

==> files/05.2_spark_results.tex <==
\begin{figure}[!htbp]
  \begin{center}
    \begin{tabular}{lrrrr}
      \toprule
                & \(\not\equiv\) & \(\equiv\) & \unknown & Total \\
      \midrule
      \sqlSolver &                & 88         &         & 88    \\
      SPES      &                & 73         &         & 88    \\
      cvc5 sets & 6 (2)          & 77         & 5       & 88    \\
      cvc5 bags & 7 (2)          & 53         & 28      & 88    \\
      \bottomrule
    \end{tabular}
  \end{center}
  \caption{Spark benchmarks. There are actually two inequivalent queries here. 
  The other are bogus.}
  \label{fig:spark_results}
\end{figure}

==> files/basic.tex <==
\subsection{Signature $\Sigma_{Bags}$}
\subsection{Types}
\begin{itemize} 
\item \ms $(\alpha)$
\item Int 
\end{itemize}
\subsection{Bag symbols}
\begin{itemize}
\item Multiplicity $\textbf{m}: \alpha \times \ms(\alpha) \rightarrow \text{Int}$ 
\item Empty Bag $\textbf{empty}: \ms(\alpha)$ 
\item Disjoint union $\uplus: \ms(\alpha) \times \ms(\alpha) \rightarrow \ms(\alpha)$
\item Union $\cup: \ms(\alpha) \times \ms(\alpha) \rightarrow \ms(\alpha)$
\item Intersection $\cap: \ms(\alpha) \times \ms(\alpha) \rightarrow \ms(\alpha)$
\item Difference Subtract $\setminus: \ms(\alpha) \times \ms(\alpha) \rightarrow \ms(\alpha)$
\item Difference Remove $\setminus \setminus: \ms(\alpha) \times \ms(\alpha) \rightarrow \ms(\alpha)$
\item $\textbf{setof}: \ms(\alpha) \rightarrow \ms(\alpha)$ 
\item $\textbf{singleton}: \alpha \rightarrow \ms(\alpha)$  
\end{itemize}

\subsection{$\Sigma_{M}$ constraints}

\begin{itemize}
\item Bag equality $\approx: \ms(\alpha) \times \ms(\alpha) \rightarrow \text{Bool}$ 
\item Bag disequality $\not\approx: \ms(\alpha) \times \ms(\alpha) \rightarrow \text{Bool}$ 
\item Bag subset $\subseteq: \ms(\alpha) \times \ms(\alpha) \rightarrow \text{Bool}$ 
\\textbf{m}ltiset  $(A \subseteq B) \equiv (A \cap B \approx A)$

\item Multiplicity constraints $\textbf{m}(a, A)= x$  where $x$ is a variable of type Int. 
\item Multiplicity constraints $\textbf{m}(a, A) \neq x$ where $x$ is a variable of type Int. 
\end{itemize}



\subsection{Translating Bag constraints to Linear Integer  Arithmetic constraints}

\subsection*{Notation}

\begin{enumerate}

\item $A, B, C, \cdots$ denote bag variables.
\item $a, b, c, \cdots$ denote bag element variables.
\item $x_{(a, A)}$ denote the integer variable for the multiplicity of element $a$ in Bag $A$
\item $v_1, v_2, v_3, \cdots$ denote integer variables. 
% \item $\mathbb{B}$ denotes the set of  Bag constraints after purification\footnote{Variable abstraction phase in Nelson-Oppen method \cite{nelson}}. 
% Examples $A = B \cup C, A \neq B \uplus C$ where $A, B, C$ are Bag variables. 
\item $\mathbb{E}$ denotes the set of element constraints 
(either equality or disequality) after purification. Examples $a = b, c \neq d$ where $a,b$ are element variables of the same type, and $c,d $ are element variables of the same type. 

\item $\mathbb{S}$ denotes the set of the equality constraints of the shared interface between multiplicities and integer variables. $\mathbb{S} = \lbrace \textbf{m}(a,A) \approx x_{(a,A)} \rbrace$. 

\item $\mathbb{I}$ denotes the set of integer constraints after purification. Examples $x_{(a,A)} \approx v_1,x_{(a,A)} \approx \max(x_{(a,B)}, x_{(a,C)}),x_{(a,A)} \not\approx x_{(a,B)} + x_{(a,C)}$.

\item $T_{\mathbb{B}}$ denotes the set of terms in $\mathbb{B}$ (bag terms).

\item $T_{\mathbb{E}}$ denotes the set of terms in $\mathbb{E}$ (element terms).

\item $T_{\mathbb{S}}$ denotes the set of terms in $\mathbb{S}$ (shared interface terms).

\item $T_{\mathbb{I}}$ denotes the set of terms in $\mathbb{I}$ (integer terms).



\item \begin{align*}
\mathbb{B}^* = &\lbrace A \approx B \; \vert \; A, B \in T_{\mathbb{B}}, \mathbb{B} \models A \approx B \rbrace \; \cup \\
 &\lbrace A \not\approx B \; \vert \; A, B \in T_{\mathbb{B}}, \mathbb{B} \models A \approx A', B \approx B' \text{ for some } A' \not\approx B' \in \mathbb{B} \rbrace \;
\end{align*}

\item \begin{align*}
\mathbb{E}^* = &\lbrace a \approx b \; \vert \; a, b \in T_{\mathbb{E}}, \mathbb{E} \models a \approx b \rbrace \; \cup \\
 &\lbrace a \not\approx b \; \vert \; a, b \in T_{\mathbb{E}}, \mathbb{E} \models a \approx a', b \approx b' \text{ for some } a' \not\approx b' \in \mathbb{E} \rbrace \;   
\end{align*}

\item \begin{align*}
\mathbb{I}^* = 
 &\lbrace x \approx y \; \vert \; x, y \in T_{\mathbb{I}}, \mathbb{I} \models x \approx   y \rbrace \;  \cup \\
 &\lbrace x \not \approx y \; \vert \; x, y \in T_{\mathbb{I}}, 
 \mathbb{I} \models x \approx x', y \approx y' \text{ for some } x' \not\approx y' \in \mathbb{I} \rbrace  
\end{align*}


\item Left-associative operator $\triangleleft$ : Constraints $\times$ constraint $\rightarrow$ Constraints
\begin{align*}
\mathbb{I} \triangleleft (l)= \begin{cases}
\mathbb{I} &\text{ if } l \in C^*\\
C \cup \lbrace l \rbrace  &\text{ otherwise }
\end{cases}
\end{align*}
\end{enumerate}

\subsection{Translating Bag constraints to Linear Integer  Arithmetic constraints}


\subsection*{Bag equality with multiplicity terms}

\begin{prooftree}
\AxiomC{$A \approx B \in \mathbb{B}^*$}
\AxiomC{$\textbf{m}(a, A) \in T_\mathbb{S}$ or $\textbf{m}(a, B) \in T_{\mathbb{S}}$}
\AxiomC{$x_{(a, A)} = x_{(a, B)} \not\in \mathbb{I}^*$}   
\TrinaryInfC{\small \stackanchor
{$\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)
\triangleleft \left( \textbf{m}(a, B) = x_{(a, B)} \right)$}
{$\mathbb{S}:= \mathbb{S},\mathbb{I}:= \mathbb{I} \triangleleft \left( x_{(a, A)} = x_{(a, B)} \right) $  }}
\end{prooftree}



\subsection*{Bag disequality}
\begin{prooftree}
\AxiomC{$A \not\approx B \in \mathbb{B}$}
\AxiomC{$\not\exists e \text{ such that }  x_{(e, A)} \neq x_{(e, B)}\in \mathbb{I}^*$}  
\BinaryInfC{
\small
$
\begin{matrix*}[l]
\mathbb{S}:= \mathbb{S} \triangleleft \left( \textbf{m}(a, A) \approx  x_{(a, A)} \right) \triangleleft \left(\textbf{m}(a, B) \approx x_{(a, B)} \right) \\ \mathbb{I}:= \mathbb{I} \triangleleft x_{(a, A)} \not \approx x_{(a, B)} \end{matrix*}$ for some fresh variable $a$}

\end{prooftree}

\subsection*{Bag disequality unsat}
\begin{prooftree}
\AxiomC{$A \not\approx A \in \mathbb{B}^*$} 
\UnaryInfC{unsat}
\end{prooftree}


\subsection*{Empty Bag}

\begin{prooftree}
\AxiomC{$A \approx \textbf{empty}(\alpha) \in \mathbb{B}^*$} 
\AxiomC{$\textbf{m}(a, A) \in T_{\mathbb{S}}$} 
\BinaryInfC{$\mathbb{I}:= \mathbb{I} \triangleleft \left( x_{(a, A)} =  0 \right)$}
\end{prooftree}


\subsection*{Union}

\begin{prooftree}
\AxiomC{$A \approx B \cup C \in \mathbb{B}$} 
\AxiomC{$\textbf{m}(a, A) \in T_{\mathbb{S}}$ or $\textbf{m}(a, B) \in T_{\mathbb{S}}$ or $\textbf{m}(a, C) \in T_{\mathbb{S}}$} 
\BinaryInfC{\small \stackanchor{$\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)
\triangleleft \left( \textbf{m}(a, B) = x_{(a, B)} \right)
\triangleleft \left( \textbf{m}(a, C) = x_{(a, C)} \right)$}
{$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a, A)} = \textbf{max}(x_{(a, B)} , x_{(a, C)})\right)  $}}
\end{prooftree}


\subsection*{Intersection}
\begin{prooftree}
\AxiomC{$A \approx B \cap C \in \mathbb{B}$} 
\AxiomC{$\textbf{m}(a, A) \in T_{\mathbb{S}}$ or $\textbf{m}(a, S) \in T_{\mathbb{S}}$ or $\textbf{m}(a, C) \in T_{\mathbb{S}}$} 
\BinaryInfC{\small \stackanchor{$\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)
\triangleleft \left( \textbf{m}(a, B) = x_{(a, B)} \right)
\triangleleft \left( \textbf{m}(a, C) = x_{(a, C)} \right)$}
{$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a, A)} = \textbf{min}(x_{(a, B)} , x_{(a, C)})\right)  $}}
\end{prooftree}

\subsection*{Difference Subtract}
\begin{prooftree}
\AxiomC{$A \approx B \setminus C \in \mathbb{B}$} 
\AxiomC{$\textbf{m}(a, A) \in T_{\mathbb{S}}$ or $\textbf{m}(a, S) \in T_{\mathbb{S}}$ or $\textbf{m}(a, C) \in T_{\mathbb{S}}$} 
\BinaryInfC{\small \stackanchor
{$\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)
\triangleleft \left( \textbf{m}(a, B) = x_{(a, B)} \right)
\triangleleft \left( \textbf{m}(a, C) = x_{(a, C)} \right)$}
{$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a, A)} = \textbf{ite}(x_{(a, B)} \leq x_{(a, C)}, 0, x_{(a, B)}- x_{(a, C)}) \right)  $}}
\end{prooftree}


\subsection*{Difference Remove}
\begin{prooftree}
\AxiomC{$A \approx B {{\setminus\setminus C}} \in \mathbb{B}$}
\AxiomC{$\textbf{m}(a, A) \in T_{\mathbb{S}}$ or $\textbf{m}(a, S) \in T_{\mathbb{S}}$ or $\textbf{m}(a, C) \in T_{\mathbb{S}}$}  
\BinaryInfC{\small \stackanchor
{$\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)
\triangleleft \left( \textbf{m}(a, B) = x_{(a, B)} \right)
\triangleleft \left( \textbf{m}(a, C) = x_{(a, C)} \right)$}
{$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a, A)} = \textbf{ite}(x_{(a, C)} = 0,  x_{(a, B)}, 0 ) \right)  $}}

\end{prooftree}


\subsection*{setof}
\begin{prooftree}
\AxiomC{$A \approx \textbf{setof } B \in \mathbb{B}$}
\AxiomC{$\textbf{m}(a, A) \in T_{\mathbb{S}}$ or $\textbf{m}(a, B) \in T_{\mathbb{S}}$} 

\BinaryInfC{\small \stackanchor
{$\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)
\triangleleft \left( \textbf{m}(a, B) = x_{(a, B)} \right)
$}{$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a, A)} = \textbf{ite}(1 \leq x_{(a, B)},1, 0 ) \right) $}}
\end{prooftree}

\subsection*{singleton1}
\begin{prooftree}
\AxiomC{$A \approx \textbf{singleton}(a) \in \mathbb{B} $} 
\AxiomC{$x_{(a, A)}  \approx 1 \not\in \mathbb{I}^*$} 
\BinaryInfC{\small $\mathbb{S}:= \mathbb{S} 
\triangleleft \left( \textbf{m}(a, A) = x_{(a, A)} \right)$, $\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a, A)} \approx 1 \right) $}
\end{prooftree}

\subsection*{singleton2}
\begin{prooftree}
\AxiomC{$A \approx \textbf{singleton}(a) \in \mathbb{B} $} 
\AxiomC{$\textbf{m}(b, A) \in T_\mathbb{S}$}
\AxiomC{$x_{(b, A)} \not\approx 0 \in \mathbb{I}^*$}
\AxiomC{$b \approx a \not\in \mathbb{E}^*$}  
\QuaternaryInfC{$\mathbb{E}:= \mathbb{E} \triangleleft \left( b \approx a \right)$,$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(b, A)} \approx 1 \right) $}
\end{prooftree}

\subsection*{multiplicity variables}
\begin{prooftree}
\AxiomC{$x_{(a,A)} \in T_{\mathbb{S}} $} 
\AxiomC{$x_{(a,A)} \geq 0 \not\in {\mathbb{I}^*}$}
\BinaryInfC{$\mathbb{I}:= \mathbb{I} \triangleleft \left(x_{(a,A)} \geq 0 \right) $}
\end{prooftree}


\subsection{Constructing a model}

A model $M$ obtained from the arithmetic solver would assign values to multiplicity variables $M=\lbrace \left(x_{(a, A)}, v_{\textbf{m}(a, A)} \right)\vert \; a : \alpha_A, A : \text{Bag}(\alpha_A) \rbrace$. To construct a model $M'$ for the Bag constraints, we start from an empty model $M' = \phi$, and for each Bag variable $A$, there are 2 cases: 

\begin{enumerate}
\item There is no variable for $A$ in $M$. In this case $M' = M' \; \cup \; (A, \textbf{ empty}(\alpha_A))$.

\item $M$ has variables $(x_a, v_a), (x_b, v_b), \cdots, (x_z, v_z)$ where $a, b, \cdots, z$ are distinct elements. In this case, 
\begin{align*}
M' &= M' \; \cup \; (A, \lbrace \underbrace{x_a, x_a, \cdots, x_a}_{v_a}, 
\underbrace{x_b, x_b, \cdots, x_b}_{v_b}, \cdots, \underbrace{x_z, x_z, \cdots, x_z}_{v_z} \rbrace) \\
&= M' \; \cup \; (A, \biguplus\limits_{i = 1}^{v_a} \lbrace x_a \rbrace \uplus 
\biguplus\limits_{i = 1}^{v_b}\lbrace x_b \rbrace\uplus \cdots \uplus \biguplus\limits_{i = 1}^{v_z}\lbrace x_z \rbrace )
\end{align*}


\end{enumerate}

\subsection{Examples}


The following example is from ``Combining multisets with integers". We want to show the following formula is unsatisfiable
\begin{align*}
A \uplus B \not\approx (A \cup B) \uplus (A \cap B).
\end{align*}

\begin{enumerate}
\item We purify the formula to get :
\small
\begin{align*}
\mathbb{B} &= \lbrace C \approx A \uplus B, D \approx A \cup B, E \approx A \cap B, F \approx D \uplus E, 
 C \not \approx F  \rbrace
\end{align*}
\normalsize
\item We apply the bag disequality rule for $C \neq D$:
\small
\begin{align*}
\mathbb{B} &= \lbrace C \approx A \uplus B, D \approx A \cup B, E \approx A \cap B, F \approx D \uplus E, 
 C \not \approx F  \rbrace \\
\mathbb{S} &= \lbrace \textbf{m}(a, C) \approx  x_{(a, C)}  , \textbf{m}(a, F) \approx x_{(a, F)} \rbrace \\
\mathbb{I} &= \lbrace x_{(a, C)} \not\approx  x_{(a, F)}\rbrace
\end{align*}
\normalsize
where $a$ is a fresh element variable. 

\item We apply the disjoint union rule for $C \approx A \uplus B$ :
\small
\begin{align*}
\mathbb{B} &= \lbrace C \approx A \uplus B, D \approx A \cup B, E \approx A \cap B, F \approx D \uplus E, 
 C \not \approx F  \rbrace \\
\mathbb{S} &= \lbrace \textbf{m}(a, C) \approx  x_{(a, C)}  , \textbf{m}(a, F) \approx x_{(a, F)},  \textbf{m}(a, A) \approx  x_{(a, A)} ,  \textbf{m}(a, B) \approx  x_{(a, B)}  \rbrace \\
\mathbb{I} &= \lbrace x_{(a, C)} \not\approx  x_{(a, F)},  x_{(a, C)} \approx  x_{(a, A)} + x_{(a, B)} \rbrace
\end{align*}
\normalsize


\item We apply the union rule for $D \approx A \cup B$ :
\small
\small
\begin{align*}
\mathbb{B} &= \lbrace C \approx A \uplus B, D \approx A \cup B, E \approx A \cap B, F \approx D \uplus E, 
 C \not \approx F  \rbrace \\
\mathbb{S} &= \begin{Bmatrix*}[l] 
\textbf{m}(a, C) \approx  x_{(a, C)}  , \textbf{m}(a, F) \approx x_{(a, F)},  \textbf{m}(a, A) \approx  x_{(a, A)} ,    \\
\textbf{m}(a, B) \approx  x_{(a, B)}, \textbf{m}(a, D) \approx  x_{(a, D)}
\end{Bmatrix*}  \\
\mathbb{I} &= \lbrace x_{(a, C)} \not\approx  x_{(a, F)},  x_{(a, C)} \approx  x_{(a, A)} + x_{(a, B)}, x_{(a, D)} = \textbf{max}(x_{(a, A)} , x_{(a, B)}) \rbrace 
\end{align*}
\normalsize

\item We apply the intersection rule for $E \approx A \cap B$ :
\small
\begin{align*}
\mathbb{B} &= \lbrace C \approx A \uplus B, D \approx A \cup B, E \approx A \cap B, F \approx D \uplus E, 
 C \not \approx F  \rbrace \\
\mathbb{S} &= \begin{Bmatrix*}[l] 
\textbf{m}(a, C) \approx  x_{(a, C)}  , \textbf{m}(a, F) \approx x_{(a, F)},  \textbf{m}(a, A) \approx  x_{(a, A)} ,    \\
\textbf{m}(a, B) \approx  x_{(a, B)}, \textbf{m}(a, D) \approx  x_{(a, D)},
\textbf{m}(a, E) \approx  x_{(a, E)}
\end{Bmatrix*}  \\
\mathbb{I} &= \begin{Bmatrix*}[l] 
 x_{(a, C)} \not\approx  x_{(a, F)} ,&  x_{(a, C)} \approx  x_{(a, A)} + x_{(a, B)}, \\
 x_{(a, D)} = \textbf{max}(x_{(a, A)} , x_{(a, B)}),&
 x_{(a, E)} = \textbf{min}(x_{(a, A)} , x_{(a, B)}) \end{Bmatrix*}  
\end{align*}
\normalsize

\item We apply the disjoint union rule for $F \approx D \uplus E$ :
\small
\begin{align*}
\mathbb{B} &= \lbrace C \approx A \uplus B, D \approx A \cup B, E \approx A \cap B, F \approx D \uplus E, 
 C \not \approx F  \rbrace \\
\mathbb{S} &= \begin{Bmatrix*}[l] 
\textbf{m}(a, C) \approx  x_{(a, C)}  , \textbf{m}(a, F) \approx x_{(a, F)},  \textbf{m}(a, A) \approx  x_{(a, A)} ,    \\
\textbf{m}(a, B) \approx  x_{(a, B)}, \textbf{m}(a, D) \approx  x_{(a, D)},
\textbf{m}(a, E) \approx  x_{(a, E)}
\end{Bmatrix*}  \\
\mathbb{I} &= \begin{Bmatrix*}[l] 
 x_{(a, C)} \not\approx  x_{(a, F)} ,&  x_{(a, C)} \approx  x_{(a, A)} + x_{(a, B)}, \\
 x_{(a, D)} = \textbf{max}(x_{(a, A)} , x_{(a, B)}),&
 x_{(a, E)} = \textbf{min}(x_{(a, A)} , x_{(a, B)})  \\
 x_{(a, F)} \approx  x_{(a, D)} + x_{(a, E)} 
 \end{Bmatrix*}  
\end{align*}
\normalsize

\end{enumerate}

The constraints in $\mathbb{I}$ now can be sent to the liner arithmetic solver which will return unsat. 

